PolicyCleanse: Backdoor Detection and Mitigation in Reinforcement Learning

While real-world applications of reinforcement learning are becoming popular, the security and robustness of RL systems are worthy of more attention and exploration. In particular, recent works have revealed that, in a multi-agent RL environment, backdoor trigger actions can be injected into a victim agent (a.k.a. Trojan agent), which can result in a catastrophic failure as soon as it sees the backdoor trigger action. To ensure the security of RL agents against malicious backdoors, in this work, we propose the problem of Backdoor Detection in a multi-agent competitive reinforcement learning system, with the objective of detecting Trojan agents as well as the corresponding potential trigger actions, and further trying to mitigate their Trojan behavior. In order to solve this problem, we propose PolicyCleanse that is based on the property that the activated Trojan agents accumulated rewards degrade noticeably after several timesteps. Along with PolicyCleanse, we also design a machine unlearning-based approach that can effectively mitigate the detected backdoor. Extensive experiments demonstrate that the proposed methods can accurately detect Trojan agents, and outperform existing backdoor mitigation baseline approaches by at least 3% in winning rate across various types of agents and environments.

==> tab_t.tex <==
\begin{table}[!t]
    \centering
\setlength\tabcolsep{5pt}
    \resizebox{\linewidth}{!}{
        \begin{tabular}{cccccc}
    \toprule
    \multirow{2}{*}{\bf HParams}  &%\multicolumn{4}{c}{\begin{tabular}[c]{@{}l@{}} \bf Game \end{tabular}} \\  &
    \bf Run-To-Goal & \bf Run-To-Goal & \bf You-Shall-Not-Pass
                        & \bf Sumo      \\
    & \bf (Ants) &\bf (Humans) & & \bf (Humans) \\
    \midrule 
    $T_r$ & 70 &  Falling Down & Falling Down & Falling Down
\\
             $N$ & 40 & 10& 10& 10
           
             
             
\\ \bottomrule
    \end{tabular}}
    \centering
    \caption{\small The hyperparameters for each game.}% For each attack approach, we build 60 infected models for each task.}
     \label{table:hyperp}
  
\end{table}
